Self-Guided Multiple Instance Learning for Weakly Supervised Disease Classification and Localization in Chest Radiographs

The lack of fine-grained annotations hinders the deployment of automated diagnosis systems, which require human-interpretable justification for their decision process. In this paper, we address the problem of weakly supervised identification and localization of abnormalities in chest radiographs. To that end, we introduce a novel loss function for training convolutional neural networks increasing the \emph{localization confidence} and assisting the overall \emph{disease identification}. The loss leverages both image- and patch-level predictions to generate auxiliary supervision. Rather than forming strictly binary from the predictions as done in previous loss formulations, we create targets in a more customized manner, which allows the loss to account for possible misclassification. We show that the supervision provided within the proposed learning scheme leads to better performance and more precise predictions on prevalent datasets for multiple-instance learning as well as on the NIH~ChestX-Ray14 benchmark for disease recognition than previously used losses.

==> Images/Experiments/Results/Second_dataset_experiments.tex <==
\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        Architecture & \diagbox[width=7.5em]{Method}{Disease}& Atelectasis  & Cardiomegaly  &  Consolidation &  Edema & Effusion  & Emphysema  & Fibrosis & Hernia  & Infiltrate  &  Mass &  Nodule & \makecell{Pleural \\ Thickening}   & Pneumonia  & Pneumothorax  & Mean     \\\hline
         \multirow{3}{*}{ResNet}&Wang et al.*&&&&&&&&&&&&&&& \\\hline
         &Li et al.*&&&&&&&&&&&&&&& \\\hline
         &Liu et al.*&&&&&&&&&&&&&&& \\\hline
         \multirow{3}{*}{DenseNet}&HCT(Ours)&&&&&&&&&&&&&&& \\\hline
         &&&&&&&&&&&&&&& \\\hline
         &&&&&&&&&&&&&&& \\\hline

         

    \end{tabular}%
    }
    \caption{Ablation study on the effect of model parts on the classification performance. Here, 70\% of all images were used for training with no bounding box annotations available. Evaluations were performed on the official test split containing 20\% of all images.}
    \label{tab:abl_classification}
\end{table}

==> Images/Experiments/Results/auprc.tex <==
\vspace{-30pt}
\begin{table}[h]
\scriptsize
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        
        \diagbox[width=7.5em]{Method}{Pathologies}& At.  & Card.  &  Cons. &  Ed. & Eff.  & Emph.  & Fib. & Hernia  & Inf.  &  Mass &  Nod. & Pl.   & Pn.  & Pt.  & Mean     \\\hline\hline
         ResNet-50+SGL&0.36&0.35& 0.17&0.19&0.54& 0.47& 0.11&0.43&0.41& 0.35&0.29&0.18&0.06&0.49& 0.31 \\\hline
    \end{tabular}%
    }
    \label{tab:class}
\end{table}
\vspace{-25pt}

==> Images/Experiments/ablation/Images_ablation_epochs.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth,height=0.4\textheight]{example-image-a}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> Images/Experiments/ablation/plots_ablation.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{.3\linewidth}
    \centering\includegraphics[width=\textwidth]{example-grid-100x100pt}
    \caption{This is a sub-caption. This is a sub-caption. This is a sub-caption}
  \end{subfigure}
  \begin{subfigure}[t]{.3\linewidth}
    \centering\includegraphics[width=\textwidth]{example-grid-100x100pt}
    \caption{This is a sub-caption.}
  \end{subfigure}
  \begin{subfigure}[t]{.3\linewidth}
    \centering\includegraphics[width=\textwidth]{example-grid-100x100pt}
    \caption{This is a sub-caption. This is a sub-caption.}
  \end{subfigure}
    
    \caption{Bar Plot Ablation of different prediction value distributions over several different epochs with corresponding avg auc.}
    \label{fig:my_label}
\end{figure}

==> Images/Experiments/ablation/tables_ablation_design.tex <==
\begin{subtable}[t]{0.5\linewidth}

    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|ccc|c|c|}
    \hline
        Method & Choice 1 & Choice 2 & Choice 3 & AUC & CorLoc \\
    \hline
        tmp & \checkmark & \checkmark & \checkmark & 0.0 & 0.0 \\
        \hline
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{subtable}


==> Images/Experiments/ablation/tables_ablation_hyper.tex <==
\begin{subtable}[t]{0.5\linewidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|ccc|c|c|}
    \hline
        Method & Choice 1 & Choice 2 & Choice 3 & AUC & CorLoc \\
    \hline
        tmp & \checkmark & \checkmark & \checkmark & 0.0 & 0.0 \\
        \hline
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{subtable}


==> Sections/rebuttal.tex <==
We thank the reviewers for their thoughtful remarks and feedback.

\newsec{Reviewer 1} 
\newsec{Choice of $\delta$} We tested different values of $\delta$ on MNIST-Bags, but did not find major differences in performance, apart from $\delta=0.5$ performing noticeably worse. We found this is also partly due to the rescaling component, which indirectly adapts the actual threshold to the present data. We originally integrated the rescaling to offset prediction bias (particularly visible in the middle columns of~Fig.~7). We will integrate the impact of the rescaling component into the ablation study. We did not investigate a dynamic choice of delta, however, we agree that this could make the method more flexible.

\newsec{Choice  of $\alpha$}
The motivation of the factor~$\alpha$ is to weigh the loss based on the overall confidence of the network, such that the loss has higher weight the better it differentiates between high and low predictions. If the network is unable to differentiate the pseudo supervision should be given no weight, but the more confident the predictions get the stronger the pseudo-supervision is applied. We choose the median over the mean to potentially capture the full range of [0,1]. 
We show the impact of the weighing factor $\alpha$ in Fig. 5a.

\newsec{Choice of $\lambda$}We choose parameter $\lambda$ to accommodate for the data imbalance existing within the dataset. In ChestXRay-14 exists a massive imbalance between positive and negative bags. Therefore, we chose to set $\lambda$ to 20 to offset this imbalance as otherwise the loss would mainly be dominated by $M^c_{i,j}=0$.

\noindent We agree with Reviewer 1 that parts of SGL's formulation are not fully motivated in this paper. We will clarify the reasoning behind each component.
\newsec{Clarification regarding the FCN}
In Fig. 3, we display the common FCN setup  consisting of a backbone (i.e. ResNet-50) to extract features followed by a layer to produce predictions for the given task (i.e. 14 disease classes, 1000 ImageNet classes, etc.). We use the predictions of the final layer, which are in form of a prediction map, and feed it to our loss. This way we do not require changes on a given FCN architecture. We make sure to clarify this in Section~3.3. 

% \newsec{AUPRC Results on ChestXRay-14}
% We used evaluation metrics mentioned in related work for a fair comparison.


\newsec{Reviewer 2 and 3} 
\newsec{Cifar-10-Bags Performance}
    We agree with the reviewers that the improvements on CIFAR10 are rather marginal. We attribute this to our method using Max-Pooling to stay consistent with prior experiments. This pooling struggles to backpropagate all information visible within a sample, which poses a obstacle for any training procedure  (ie. we were unable to perform training with BIL with Max-Pooling, which lead us to apply Mean-pooling for BIL). Despite this, our method manages to consistently achieve up to double the IoU of other methods for bags with a low percentage of positive instances. Thus, we argue that it improve distinctions between pos./neg. in MIL problems.
    
\newsec{On potential uses for CXR diagnosis}
    Apart from the integration of this loss into an off-the-shelf ResNet achieving a mean AUROC of 0.831 compared to Liu~\etal's 0.826, who also integrate an additional ResNet18 and other architectural changes, we see the main strength of our method in the overall ease of use. We have shown the general applicability of our loss function on different data sets.    Thus, we assume that other prominent methods on the ChestXRay-14 dataset that also rely on FCNs can benefit from our loss function as this might further improve not only CXR classification but also their interpretability. 
    




% In a MIL-scenario, we assume that we are usually faced with a multitude of negative instances and a few positive instances. 
% The motivation of the factor $\alpha$ is to weigh the loss based on the overall confidence of the network, such that the loss has higher weight the more confident the network is with its predictions. We say a network is confident the more distinct the network differentiates between high and low predictions. In an ideal scenario under the assumption that a bag contains mostly negative instance and a few positive instances the network will have a few $1$- and a large amount of $0$-predictions. Thus the median of the predictions will be $0$. We choose the median over the mean to potentially capture the full range of [0,1]. We show the impact of the weighing factor $\alpha$ in Fig. 5a).

% We apply the rescaling to adjust the networks predictions which we found in many cases to be attributable to a general bias. I.e. for classes with small amounts of positive bags the network predictions in many cases will usually default to low range of prediction scores e.g. $[0.-0.3]$. By rescaling, the network is enticed to follow guesses, which go ever-so-slightly contrary to the overall prediction distribution for positive bags. In the example mentioned by R1, we have the opposite case, where the network might generalizes predictions to a high base prediction score to minimize the overall error, which leads to likely negative instances having a $0.4$-score.  Thus, a prediction of $0.6$ is less indicative for the network in comparison to $1$ but still nudges the classifier slightly towards a positive prediction. If no rescaling would be applied the network would have no positive target for our first or nearly no negative target for latter case, with both cases going against our underlying assumption.
